Learning Zero-Shot Cooperation with Humans, Assuming Humans Are Biased

There is a recent trend of applying multi-agent reinforcement learning (MARL) to train an agent that can cooperate with humans in a zero-shot fashion without using any human data. The typical workflow is to first repeatedly run self-play (SP) to build a policy pool and then train the final adaptive policy against this pool. A crucial limitation of this framework is that every policy in the pool is optimized w.r.t. the environment reward function, which implicitly assumes that the testing partners of the adaptive policy will be precisely optimizing the same reward function as well. However, human objectives are often substantially biased according to their own preferences, which can differ greatly from the environment reward. We propose a more general framework, Hidden-Utility Self-Play (HSP), which explicitly models human biases as hidden reward functions in the self-play objective. By approximating the reward space as linear functions, HSP adopts an effective technique to generate an augmented policy pool with biased policies. We evaluate HSP on the Overcooked benchmark. Empirical results show that our HSP method produces higher rewards than baselines when cooperating with learned human models, manually scripted policies, and real humans. The HSP policy is also rated as the most assistive policy based on human feedback.

==> tables/ab_policy_2.tex <==
\begin{table}
\centering

\begin{tabular}{ccccc} 
\toprule
                                        & Pos. & Asy. Adv.   & Coor. R. & Cou. Circ.  \\ 
\midrule

\multirow{2}{*}{HSP w.o. Mep}  & 1    & 308.5\scriptsize{(4.4)}  & 157.5\scriptsize{(3.0)} & 94\scriptsize{(2.7)}      \\
                                        & 2    & 219.6\scriptsize{(15.9)} & 157.7\scriptsize{(2.5)} & 100.4\scriptsize{(1.1)}   \\ 
\hline
\multirow{2}{*}{HSP w.o. Greedy}       & 1    & 311.3\scriptsize{(8.1)}  & 139.2\scriptsize{(5.6)} & 80.1\scriptsize{(4.6)}    \\
                                        & 2    & 209.3\scriptsize{(4.0)}  & 138.5\scriptsize{(3.1)} & 88.7\scriptsize{(0.9)}    \\
\hline
\multirow{2}{*}{HSP}   & 1    & 300.3\scriptsize{(2.2)}  & 160.0\scriptsize{(2.6)} & 107.4\scriptsize{(3.5)}   \\
                                        & 2    & 217.1\scriptsize{(3.3)}  & 160.6\scriptsize{(3.3)} & 106.6\scriptsize{(3.0)}   \\ 
\bottomrule
\end{tabular}

\caption{Mean episode reward and standard deviation (over 5 seeds) on 3 layouts for different methods played with human proxy policies. The Pos. column indicates the roles played by AI policies.}
\label{tab:Average-reward-policy}
\end{table}

==> tables/ab_poolsize_2.tex <==
\begin{table}
\centering
\begin{tabular}{ccccc|ccc} 
\toprule
                         & Pos.                 & Asy. Adv.  & Coor. R.   & Cou. Circ.        & Asy. Adv.   & Coor. R.   & Cou. Circ.       \\ 
\hline
\multicolumn{1}{l}{}     & \multicolumn{1}{l}{} & \multicolumn{3}{c|}{policy pool size = 36} & \multicolumn{3}{c}{policy pool size = 72}  \\ 
\midrule
\multirow{2}{*}{FCP}     & 1                    & 282.8\scriptsize{(9.4)} & 161.3\scriptsize{(1.6)} & 95.9\scriptsize{(2.0)}        & 278.3\scriptsize{(16.0)} & 158.9\scriptsize{(0.6)} & 91.9\scriptsize{(7.5)}       \\
                         & 2                    & 203.8\scriptsize{(8.2)} & 161.0\scriptsize{(2.7)} & 92.7\scriptsize{(1.3)}        & 200.9\scriptsize{(13.2)} & 156.9\scriptsize{(4.7)} & 90.7\scriptsize{(4.8)}       \\ 
\hline
\multirow{2}{*}{MEP}     & 1                    & 291.7\scriptsize{(4.6)} & 161.8\scriptsize{(0.7)} & 108.8\scriptsize{(4.2)}       & 298.2\scriptsize{(5.4)}  & 157.3\scriptsize{(2.7)} & 104.6\scriptsize{(5.0)}      \\
                         & 2                    & 203.4\scriptsize{(2.0)} & 164.2\scriptsize{(2.1)} & 111.1\scriptsize{(0.7)}       & 207.8\scriptsize{(7.3)}  & 158.9\scriptsize{(3.0)} & 105.0\scriptsize{(2.2)}        \\ 
\hline
\multirow{2}{*}{TrajDiv} & 1                    & 289.3\scriptsize{(8.8)} & 150.8\scriptsize{(3.1)} & 60.1\scriptsize{(5.0)}     & 270.8\scriptsize{(2.5)}  & 142.5\scriptsize{(2.8)} & 70.1\scriptsize{(6.7)}       \\
                         & 2                    & 194.2\scriptsize{(0.7)} & 142.1\scriptsize{(2.3)} & 53.7\scriptsize{(12.4)} & 192.8\scriptsize{(8.7)}  & 137.3\scriptsize{(4.9)} & 63.8\scriptsize{(8.2)}       \\
\bottomrule
\end{tabular}
\caption{Average episode reward and standard deviation (over 5 seeds) on 3 layouts for different methods played with human proxy policies. The Pos. column indicates the roles played by AI policies.}
\label{tab:Average-reward-poolsize}
\end{table}

==> tables/behavior_analysis.tex <==
% \begin{table}[t]
% \vspace{-6mm}
% %\captionsetup{justification=centering}
% 	\centering
	
%     \subfloat[\label{tab:ba-fartomato}\emph{Distant Tomato}]{
% 		\begin{tabular}{ccccc}
% \hline
%               & FCP  & MEP  & TrajDiv & HSP                                  \\ \hline
% Tomato & 0.84 & 0.63 & 0.68    & {\color[HTML]{FF0000} \textbf{2.69}} \\
% Mix    & 0.37 & 0.41 & 0.44    & {\color[HTML]{3531FF} \textbf{0.19}} \\ \hline
%         \end{tabular}
% 		}
%     \subfloat[\label{tab:ba-manyorders}\emph{Many Orders}]{
% 		\begin{tabular}{ccccc}
% \hline
%               & FCP  & MEP  & TrajDiv & HSP                                  \\ \hline
% Tomato & 7.11 & 6.69 & 7.27    & {\color[HTML]{FF0000} \textbf{8.93}} \\
% Mix    & 2.24 & 1.96 & 1.80    & {\color[HTML]{FE0000} \textbf{2.35}} \\ \hline
%         \end{tabular}
% 		}
% 	\centering 
% 	%\vspace{-3mm}
% 	\caption{Average soup deliveries per episode on layout {Distant Tomato} and {Many Orders}}
%     \label{tab:ba-tomato}
% \vspace{-5mm}
% \end{table}

% \begin{table}
% \centering
% \begin{tabular}{cccccc} 
% \toprule
%                             &                 & FCP  & MEP  & TrajDiv & HSP            \\ 
% \midrule
% \multirow{2}{*}{Cou. Circ.} & Oni. Pass       &      &      &         &                \\
%                             &                 &      &      &         &                \\ 
% \hline
% \multirow{2}{*}{Dis. Toma.} & Toma. So. Deli. & 0.84 & 0.63 & 0.68    & \textbf{2.69}  \\
%                             & Mix. So. Deli.  & 0.37 & 0.41 & 0.44    & \textbf{0.19}  \\ 
% \hline
% \multirow{2}{*}{Many Ord.}  & Mid. Pot        &      &      &         &                \\
%                             & Oth. Pots       &      &      &         &                \\
% \bottomrule
% \end{tabular}
% \caption{Behavioral frequency extracted from human evaluation data.}
% \label{tab:behavior}
% \end{table}


\begin{table}
\centering
\begin{tabular}{ccccc}
\toprule
              & FCP  & MEP  & TrajDiv & HSP  \\ 
\midrule
Tomato & 0.84 & 0.63 & 0.68    & {\textbf{2.69}} \\
Mixed  & 0.37 & 0.41 & 0.44    & {\textbf{0.19}} \\ \bottomrule
\end{tabular}
\caption{Soup deliveries on {Distant Tomato}}
\label{tab:ba-fartomato}
\label{tab:behavior}
\end{table}

==> tables/behavior_analysis_far_tomato.tex <==
\begin{minipage}{\textwidth}

\begin{minipage}[t]{0.4\textwidth}
\makeatletter\def\@captype{table}
%\caption{Average deliveries per episode in \emph{Distant Tomato}}
%\label{tab:ba-fartomato}
\begin{tabular}{ccccc}
\hline
              & FCP  & MEP  & TrajDiv & HSP                                  \\ \hline
Tomato & 0.84 & 0.63 & 0.68    & {\color[HTML]{FF0000} \textbf{2.69}} \\
Mix    & 0.37 & 0.41 & 0.44    & {\color[HTML]{3531FF} \textbf{0.19}} \\ \hline
\end{tabular}
\caption{Average dish deliveries per episode in \emph{Distant Tomato}}
\label{tab:ba-fartomato}
\end{minipage}

\begin{minipage}[t]{0.4\textwidth}
\makeatletter\def\@captype{table}
%\caption{Average deliveries per episode in \emph{Many Orders}}
%\label{tab:ba-manyorders}
\begin{tabular}{ccccc}
\hline
              & FCP  & MEP  & TrajDiv & HSP                                  \\ \hline
Tomato & 7.11 & 6.69 & 7.27    & {\color[HTML]{FF0000} \textbf{8.93}} \\
Mix    & 2.24 & 1.96 & 1.80    & {\color[HTML]{FE0000} \textbf{2.35}} \\ \hline
\end{tabular}
\caption{Average dish deliveries per episode in \emph{Many Orders}}
\label{tab:ba-manyorders}
\end{minipage}
\end{minipage}




==> tables/behavior_analysis_many_orders.tex <==
\begin{table}[]
\caption{Average deliveries per episode in \emph{Many Orders}}
\label{tab:my-table}
\begin{tabular}{ccccc}
\hline
              & FCP  & MEP  & TrajDiv & HSP                                  \\ \hline
Tomato Dishes & 7.11 & 6.69 & 7.27    & {\color[HTML]{FF0000} \textbf{8.93}} \\
Mix Dishes    & 2.24 & 1.96 & 1.80    & {\color[HTML]{FE0000} \textbf{2.35}} \\ \hline
\end{tabular}
\end{table}

==> tables/human_1.tex <==

\begin{table}[ht]
\begin{tabular}{cccccc}
\toprule
                     & Asym. Adv.           & Coor. Ring           & Coun. Circ.         & Dis. Toma.        & Many Ord.             \\ \midrule
FCP+$H_{True}$            & \textbf{330.2}\scriptsize{(37.57)} & 182.9\scriptsize{(21.52)}          & 123.2\scriptsize{(29.04)}          & 347.1\scriptsize{(60.35)}                & 316.8\scriptsize{(60.13)}          \\
MEP+$H_{True}$            & 326.9\scriptsize{(43.04)}          & \textbf{188.5}\scriptsize{(24.94)} & 135.7\scriptsize{(27.86)}          & 336.5\scriptsize{(64.19)}                & 320.6\scriptsize{(51.84)}          \\
TrajDiv+$H_{True}$        & 323.6\scriptsize{(46.59)}          & 180.7\scriptsize{(30.13)}          & 108.7\scriptsize{(28.82)}          & 331.4\scriptsize{(65.87)}                & 323.5\scriptsize{(61.35)}          \\
HSP+$H_{True}$            & 327.1\scriptsize{(42.82)}          & 187.2\scriptsize{(31.94)}          & \textbf{156.6}\scriptsize{(26.13)} & \textbf{358.0}\scriptsize{(46.70)}       & \textbf{382.5}\scriptsize{(55.24)} \\ 
\bottomrule
\end{tabular}
\caption{Average reward per episode in each layout with human players}
\label{tab:Average-reward-human}
\end{table}

==> tables/human_1_warmup.tex <==
\begin{table}[ht]
\begin{tabular}{cccccc}
\toprule
                     & Asy. Adv.           & Coor. Ring           & Coun. Circ.         & Dis. Toma.         & Many Ord.             \\
\midrule
FCP+$H_{True}$            & \textbf{0.101}\scriptsize{(0.032)}          & 0.056\scriptsize{(0.017)}          & 0.045\scriptsize{(0.013)}          & 0.105\scriptsize{(0.037)}          & 0.120\scriptsize{(0.030)}          \\
MEP+$H_{True}$            & 0.097\scriptsize{(0.032)}          & 0.056\scriptsize{(0.022)}          & 0.043\scriptsize{(0.013)}          & 0.107\scriptsize{(0.038)}          & 0.105\scriptsize{(0.030)}          \\
TrajDiv+$H_{True}$        & 0.100\scriptsize{(0.026)} & 0.060\scriptsize{(0.016)}          & 0.042\scriptsize{(0.013)}          & 0.110\scriptsize{(0.032)}          & 0.116\scriptsize{(0.027)}          \\
HSP+$H_{True}$            & 0.094\scriptsize{(0.036)}          & \textbf{0.061}\scriptsize{(0.023)} & \textbf{0.054}\scriptsize{(0.016)} & \textbf{0.151}\scriptsize{(0.021)} & \textbf{0.131}\scriptsize{(0.037)} \\ 
\bottomrule
\end{tabular}
\caption{Average reward per step in each layout with human players in warmup stage}
\label{tab:Average-reward-human-warmup}
\end{table}

==> tables/human_2.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccc} 
\toprule
                                 & Pos. & Asy. Adv.           & Coor. Ring           & Cou. Circ.         \\ 
\midrule
\multirow{2}{*}{FCP+$H_{True}$}     & 1       & \textbf{339.3}\scriptsize{(38.17)} & 185.0\scriptsize{(19.73)}         & 127.7\scriptsize{(28.14)}\\ 
% \cline{2-7}
                                 & 2       & 321.3\scriptsize{(34.80)}          & 180.7\scriptsize{(22.98)}          & 118.3\scriptsize{(29.20)}  \\ 
\hline
\multirow{2}{*}{MEP+$H_{True}$}     & 1       & 329.7\scriptsize{(45.97)}         & \textbf{193.3}\scriptsize{(22.11)} & 136.9\scriptsize{(27.00)} \\ 
% \cline{2-7}
                                 & 2       & \textbf{324.2}\scriptsize{(39.93)}          & 183.6\scriptsize{(26.75)}          & 134.5\scriptsize{(28.63)}\\ 
\hline
\multirow{2}{*}{TrajDiv+$H_{True}$} & 1       & 329.0\scriptsize{(43.18)}         & 184.7\scriptsize{(28.60)}          & 112.6\scriptsize{(25.78)} \\ 
% \cline{2-7}
                                 & 2       & 318.8\scriptsize{(48.97)}          & 176.8\scriptsize{(31.33)}          & 105.0\scriptsize{(31.05)} \\ 
\hline
\multirow{2}{*}{HSP+$H_{True}$}     & 1       & 336.0\scriptsize{(35.55)}          & 185.5\scriptsize{(38.92)}         & \textbf{158.0}\scriptsize{(28.56)}\\ 
% \cline{2-7}
                                 & 2       & 318.8\scriptsize{(48.97)}         & \textbf{188.9}\scriptsize{(22.00)}           & \textbf{155.2}\scriptsize{(23.43)}    \\
\bottomrule
\end{tabular}
\caption{Average reward per episode in each layout with human players}
\label{tab:Average-reward-human}
\end{table}



==> tables/human_2_full.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccccc} 
\toprule
                                 & Pos. & Asy. Adv.           & Coor. Ring           & Cou. Circ.   & Dis. Toma.        & Many Ord.           \\ 
\midrule
\multirow{2}{*}{FCP+$H_{True}$}     & 1       & \textbf{339.3}\scriptsize{(38.17)}  & 185.0\scriptsize{(19.73)}     & 127.7\scriptsize{(28.14)}                                       & \textbf{351.3}\scriptsize{(82.25)}  & 312.4\scriptsize{(58.73)}\\ 
% \cline{2-7}
                                    & 2       & 321.3\scriptsize{(34.80)}          & 180.7\scriptsize{(22.98)}      &118.3\scriptsize{(29.20)}    & \textbf{320.5}\scriptsize{(66.49)}   &321.3\scriptsize{(61.12)} \\ 
\hline
\multirow{2}{*}{MEP+$H_{True}$}     & 1       & 329.7\scriptsize{(45.97)}         & \textbf{193.3}\scriptsize{(22.11)} & 136.9\scriptsize{(27.00)}                                     & 341.9 \scriptsize{(65.07)}  & 322.0\scriptsize{(50.53)}\\ 
% \cline{2-7}
                                 & 2       & \textbf{324.2}\scriptsize{(39.93)}          & 183.6\scriptsize{(26.75)}  &134.5\scriptsize{(28.63)}     & 313.9\scriptsize{(78.29)} & 319.2\scriptsize{(52.98)}\\ 
\hline
\multirow{2}{*}{TrajDiv+$H_{True}$} & 1       & 329.0\scriptsize{(43.18)}         & 184.7\scriptsize{(28.60)}          & 112.6\scriptsize{(25.78)}                                               & 327.1\scriptsize{(71.04)} & 312.9\scriptsize{(62.82)}\\ 
% \cline{2-7}
                                 & 2       & 318.8\scriptsize{(48.97)}          & 176.8\scriptsize{(31.33)}          & 105.0\scriptsize{(31.05)}            & 316.0\scriptsize{(77.65)} & 334.2\scriptsize{(57.99)}\\
\multirow{2}{*}{HSP+$H_{True}$}     & 1       & 336.0\scriptsize{(35.55)}    & 185.5\scriptsize{(38.92)}    &\textbf{158.0}\scriptsize{(28.56)}                                       & 331.6\scriptsize{(61.33)} & \textbf{384.3}\scriptsize{(47.50)}\\ 
% \cline{2-7}
                                 & 2       & 318.8\scriptsize{(48.97)}  & \textbf{188.9}\scriptsize{(22.00)}  & \textbf{155.2}\scriptsize{(23.43)}   & 305.9\scriptsize{(58.61)}  & \textbf{380.7}\scriptsize{(62.27)}\\
\bottomrule
\end{tabular}
\caption{Average reward per episode in each layout with human players}
\label{tab:Average-reward-human}
\end{table}

==> tables/human_2_warmup.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccc} 
\toprule
                                 & Pos. & Asy. Adv.           & Coor. Ring           & Coun. Circ.               \\ 
\midrule
\multirow{2}{*}{FCP+$H_{True}$}     & 1       & \textbf{0.104}\scriptsize{(0.035)}   & 0.050\scriptsize{(0.017)}     & 0.047\scriptsize{(0.010)}          \\ 
% \cline{2-7}
                                 & 2       & 0.098\scriptsize{(0.027)}            & 0.060\scriptsize{(0.016)}          & 0.043\scriptsize{(0.014)} \\ 
\hline
\multirow{2}{*}{MEP+$H_{True}$}     & 1       & 0.098\scriptsize{(0.038)}        & \textbf{0.062}\scriptsize{(0.018)}          & 0.046\scriptsize{(0.011)}  \\ 
% \cline{2-7}
                                 & 2       & 0.097\scriptsize{(0.025)}            & 0.051\scriptsize{(0.024)}          & 0.040\scriptsize{(0.014)}      \\ 
\hline
\multirow{2}{*}{TrajDiv+$H_{True}$} & 1       & 0.100\scriptsize{(0.018)}         & 0.058\scriptsize{(0.021)}          & 0.048\scriptsize{(0.012)}      \\ 
% \cline{2-7}
                                 & 2       & \textbf{0.100}\scriptsize{(0.034)}          & \textbf{0.062}\scriptsize{(0.012)}   & 0.037\scriptsize{(0.012)}     \\ 
\hline
\multirow{2}{*}{HSP+$H_{True}$}     & 1       & 0.094\scriptsize{(0.039)}          & 0.061\scriptsize{(0.019)}         & \textbf{0.060}\scriptsize{(0.011)} \\ 
% \cline{2-7}
                                 & 2       & 0.095\scriptsize{(0.032)}         & 0.061\scriptsize{(0.025)}            & \textbf{0.048}\scriptsize{(0.017)}     \\
\bottomrule
\end{tabular}
\caption{Average reward per step in each layout with human players in warmup stage}
\label{tab:Average-reward-human-warmup}
\end{table}

==> tables/human_2_warmup_full.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccccc} 
\toprule
                                 & Pos. & Asy. Adv.           & Coor. Ring           & Coun. Circ.      & Dis. Toma.        & Many Ord.           \\ 
\midrule
\multirow{2}{*}{FCP+$H_{True}$}     & 1       & \textbf{0.104}\scriptsize{(0.035)}   & 0.050\scriptsize{(0.017)}     &                                                         0.047\scriptsize{(0.010)}     & 0.106\scriptsize{(0.043)}  & 0.133\scriptsize{(0.029)}  \\ 
% \cline{2-7}
                                 & 2       & 0.098\scriptsize{(0.027)}            & 0.060\scriptsize{(0.016)}          & 0.043\scriptsize{(0.014)}     & 0.094\scriptsize{(0.031)}  & 0.107\scriptsize{(0.025)} \\ 
\hline
\multirow{2}{*}{MEP+$H_{True}$}     & 1       & 0.098\scriptsize{(0.038)}        & \textbf{0.062}\scriptsize{(0.018)}          &                                               0.046\scriptsize{(0.011)}     & 0.112\scriptsize{(0.032)}  & 0.125\scriptsize{(0.029)}\\ 
% \cline{2-7}
                                 & 2       & 0.097\scriptsize{(0.025)}            & 0.051\scriptsize{(0.024)}          & 0.040\scriptsize{(0.014)}      & 0.095\scriptsize{(0.039)} & 0.090\scriptsize{(0.020)}\\ 
\hline
\multirow{2}{*}{TrajDiv+$H_{True}$} & 1       & 0.100\scriptsize{(0.018)}         & 0.058\scriptsize{(0.021)}          &                                                       0.048\scriptsize{(0.012)}      & \textbf{0.125}\scriptsize{(0.019)} & 0.132\scriptsize{(0.020)}\\ 
% \cline{2-7}
                                 & 2       & \textbf{0.100}\scriptsize{(0.034)}          & \textbf{0.062}\scriptsize{(0.012)}   & 0.037\scriptsize{(0.012)}      & 0.090\scriptsize{(0.032)}  & 0.102\scriptsize{(0.025)}\\ 
\hline
\multirow{2}{*}{HSP+$H_{True}$}     & 1       & 0.094\scriptsize{(0.039)}          & 0.061\scriptsize{(0.019)}         &                                                  \textbf{0.060}\scriptsize{(0.011)}  & 0.119\scriptsize{(0.015)}  & \textbf{0.146}\scriptsize{(0.021)}\\ 
% \cline{2-7}
                                 & 2       & 0.095\scriptsize{(0.032)}         & 0.061\scriptsize{(0.025)}            & \textbf{0.048}\scriptsize{(0.017)}  & \textbf{0.115}\scriptsize{(0.020)} & \textbf{0.116}\scriptsize{(0.042)}   \\
\bottomrule
\end{tabular}
\caption{Average reward per step in each layout with human players in warmup stage}
\label{tab:Average-reward-human-warmup}
\end{table}

==> tables/human_proxy_1.tex <==

\begin{table}[hp]
\centering
\begin{tabular}{cccc} 
\toprule
                 & Asy. Adv.           & Coor. Ring          & Coun. Circ.          \\ 
\midrule
FCP+$H_{Proxy}$     & 243.3\scriptsize{(8.8)}          & 161.1\scriptsize{(2.2)}          & 94.3\scriptsize{(1.6)}            \\
MEP+$H_{Proxy}$     & 247.5\scriptsize{(3.3)}          & \textbf{163.0}\scriptsize{(1.4)} & \textbf{109.9}\scriptsize{(2.4)}                   \\
TrajDiv+$H_{Proxy}$ & 241.7\scriptsize{(4.7)}          & 146.4\scriptsize{(2.7)}          & 56.9\scriptsize{(8.7)}                   \\
HSP+$H_{Proxy}$     & \textbf{258.7}\scriptsize{(2.8)} & 157.9\scriptsize{(2.9)}          & {107.0}\scriptsize{(3.2)}  \\
\bottomrule
\end{tabular}
\caption{Average reward per episode in each layout with human proxy}
\label{tab:Average-reward-proxy}
\end{table}

==> tables/human_proxy_2.tex <==
\begin{table}[hp]
\centering
\begin{tabular}{ccccc} 
\toprule
                                     & Pos. & Asy. Adv.           & Coor. R.          & Cou. Circ.          \\ 
\midrule
\multirow{2}{*}{FCP}     & 1    & 282.8\scriptsize{(9.4)}          & \textbf{161.3}\scriptsize{(1.6)}          & 95.9\scriptsize{(2.0)}            \\
                                     & 2    & 203.8\scriptsize{(8.2)}          & \textbf{161.0}\scriptsize{(2.7)}          & 92.7\scriptsize{(1.3)}            \\ 
\hline
\multirow{2}{*}{MEP}     & 1    & 291.7\scriptsize{(4.6)}          & \textbf{161.8}\scriptsize{(0.7)} & \textbf{108.8}\scriptsize{(4.2)}              \\
                                     & 2    & 203.4\scriptsize{(2.0)}          & \textbf{164.2}\scriptsize{(2.1)} & \textbf{111.1}\scriptsize{(0.7)}              \\ 
\hline
\multirow{2}{*}{TrajDiv} & 1    & 289.3\scriptsize{(8.8)}          & 150.8\scriptsize{(3.1)}          & 60.1\scriptsize{(5.0)}              \\
                                     & 2    & 194.2\scriptsize{(0.7)}          & 142.1\scriptsize{(2.3)}          & 53.7\scriptsize{(12.4)}              \\ 
\hline
\multirow{2}{*}{HSP}     & 1    & \textbf{300.3}\scriptsize{(2.2)} & \textbf{160.0}\scriptsize{(2.6)}          & \textbf{107.4}\scriptsize{(3.5)}  \\
                                     & 2    & \textbf{217.1}\scriptsize{(3.3)} & \textbf{160.6}\scriptsize{(3.3)}          & \textbf{106.6}\scriptsize{(3.0)}           \\
\bottomrule
\end{tabular}
\caption{Mean episode reward and standard deviation (over 5 seeds) on 3 layouts for different methods played with human proxy policies. All values within 5 standard deviation of the maximum episode return are marked in bold. The Pos. column indicates the roles played by AI policies.}
\label{tab:Average-reward-proxy}
\end{table}

==> tables/human_warmup2.tex <==
\begin{table}[ht]
\centering
\begin{tabular}{ccccccc} 
\toprule
                                 & Pos. & Asy. Adv.           & Coor. Ring           & Coun. Circ.      & Dis. Toma.        & Many Ord.           \\ 
\midrule
\multirow{2}{*}{FCP}     & 1       & \textbf{0.104}\scriptsize{(0.035)}   & 0.050\scriptsize{(0.017)}     &                                                         0.047\scriptsize{(0.010)}     & 0.106\scriptsize{(0.043)}  & 0.133\scriptsize{(0.029)}  \\ 
% \cline{2-7}
                                 & 2       & 0.098\scriptsize{(0.027)}            & 0.060\scriptsize{(0.016)}          & 0.043\scriptsize{(0.014)}     & 0.094\scriptsize{(0.031)}  & 0.107\scriptsize{(0.025)} \\ 
\hline
\multirow{2}{*}{MEP}     & 1       & 0.098\scriptsize{(0.038)}        & \textbf{0.062}\scriptsize{(0.018)}          &                                               0.046\scriptsize{(0.011)}     & 0.112\scriptsize{(0.032)}  & 0.125\scriptsize{(0.029)}\\ 
% \cline{2-7}
                                 & 2       & 0.097\scriptsize{(0.025)}            & 0.051\scriptsize{(0.024)}          & 0.040\scriptsize{(0.014)}      & 0.095\scriptsize{(0.039)} & 0.090\scriptsize{(0.020)}\\ 
\hline
\multirow{2}{*}{TrajDiv} & 1       & 0.100\scriptsize{(0.018)}         & 0.058\scriptsize{(0.021)}          &                                                       0.048\scriptsize{(0.012)}      & \textbf{0.125}\scriptsize{(0.019)} & 0.132\scriptsize{(0.020)}\\ 
% \cline{2-7}
                                 & 2       & \textbf{0.100}\scriptsize{(0.034)}          & \textbf{0.062}\scriptsize{(0.012)}   & 0.037\scriptsize{(0.012)}      & 0.090\scriptsize{(0.032)}  & 0.102\scriptsize{(0.025)}\\ 
\hline
\multirow{2}{*}{HSP}     & 1       & 0.094\scriptsize{(0.039)}          & 0.061\scriptsize{(0.019)}         &                                                  \textbf{0.060}\scriptsize{(0.011)}  & 0.119\scriptsize{(0.015)}  & \textbf{0.146}\scriptsize{(0.021)}\\ 
% \cline{2-7}
                                 & 2       & 0.095\scriptsize{(0.032)}         & 0.061\scriptsize{(0.025)}            & \textbf{0.048}\scriptsize{(0.017)}  & \textbf{0.115}\scriptsize{(0.020)} & \textbf{0.116}\scriptsize{(0.042)}   \\
\bottomrule
\end{tabular}
\caption{Average reward per step in all layouts with human players in the warmup stage.}
\label{tab:Average-reward-human-warmup}
\end{table}

==> tables/script_agent_2.tex <==

\begin{table}[ht]
\centering
\scriptsize
\begin{tabular}{cccccccccc} 
\toprule
                             & \multirow{2}{*}{Scripts} & \multicolumn{2}{c}{FCP}                   & \multicolumn{2}{c}{MEP}                     & \multicolumn{2}{c}{TrajDiv} & \multicolumn{2}{c}{HSP}                      \\ 
\cline{3-10}
                             &                          & 1                   & 2                   & 1                    & 2                    & 1           & 2             & 1                    & 2                     \\ 
\midrule
\multirow{2}{*}{Asy. Adv.}   & Oni. Pla.                & 304.0(20.8)         & 365.7(5.3)          & 295.0(25.7)          & 365.9(2.8)           & 296.5(25.2) & 350.7(8.9)    & \textbf{357.3}(2.4)  & \textbf{396.3}(17.4)  \\
                             & Oni. Pla.\&Deli.               & 364.9(2.9)          & \textbf{230.5}(3.9) & \textbf{366.8}(1.5)  & \textbf{230.3}(5.3)  & 358.2(6.0)  & 221.8(3.4)    & \textbf{371.4}(3.3)  & \textbf{229.9}(4.9)   \\ 
\hline
\multirow{2}{*}{Coor. Ring}  & Oni. Every.              & 106.0(8.7)          & 112.1(7.2)          & \textbf{124.6}(3.6)  & \textbf{123.4}(3.2)  & 115.7(11.1) & 118.1(6.7)    & \textbf{120.8}(14.3) & \textbf{121.7}(10.9)  \\
                             & Dish Every.              & 91.9(4.1)           & 97.0(3.4)           & 101.4(3.1)           & 99.0(7.3)            & 107.5(5.2)  & 107.1(5.3)    & \textbf{114.9}(7.7)  & \textbf{116.0}(7.2)   \\ 
\hline
\multirow{2}{*}{Coun. Circ.} & Oni. Every.              & 64.80(8.8)          & 62.7(9.5)           & 90.6(3.9)            & 87.4(6.2)            & 86.0(12.1)  & 78.1(13.4)    & \textbf{110.5}(3.7)  & \textbf{104.4}(3.4)   \\
                             & Dish Every.              & 57.9(5.3)           & 56.1(5.2)           & 53.5(1.1)            & 52.5(2.4)            & 59.3(2.9)   & 55.0(1.5)     & \textbf{79.3}(3.5)   & \textbf{77.8}(4.7)    \\ 
\hline
\multirow{2}{*}{Dis. Toma.}  & Toma. Pla.               & 13.5(2.6)           & 17.8(7.6)           & 25.9(17.6)           & 14.3(3.6)            & 29.6(14.1)  & 17.2(4.8)     & \textbf{277.7}(9.7)  & \textbf{278.9}(18.8)  \\
                             & Toma. Pla.\&Deli.              & 197.5(4.9)          & 158.3(7.3)          & 185.9(9.9)           & 174.8(7.4)           & 175.3(21.6) & 154.3(17.6)   & \textbf{237.2}(8.2)  & \textbf{231.9}(22.0)  \\ 
\hline
\multirow{2}{*}{Many Ord.}   & Toma. Pla.               & 285.4(19.5)         & 279.8(12.8)         & 224.1(61.2)          & 227.6(60.5)          & 263.8(10.1) & 254.6(5.7)    & \textbf{315.7}(12.1) & \textbf{319.9}(6.5)   \\
                             & Toma. Pla.\&Deli.              & \textbf{334.1}(5.6) & \textbf{324.2}(4.9) & \textbf{329.1}(12.7) & \textbf{327.2}(12.4) & 298.8(3.2)  & 292.6(1.5)    & 326.7(4.0)           & \textbf{322.3}(3.9)   \\
\bottomrule
\end{tabular}
\caption{Average reward and standard deviation in all layouts with scripted policies. All values within Within a difference of 5 from maximum reward are marked in bold. The "1" and "2" indicates the roles played by AI policies.}
\label{tab:Average-reward-script}
\end{table}

==> tables/tmp.tex <==
% \usepackage{multirow}
% \usepackage{booktabs}


\begin{table}
\centering
\caption{Average reward per step in each layout in warmup stage}
\label{tab:Average-reward-human-warmup}
\begin{tabular}{cccccccccc} 
\toprule
                               & \multirow{2}{*}{script} & \multicolumn{2}{c}{FCP} & \multicolumn{2}{c}{MEP} & \multicolumn{2}{c}{TrajDiv } & \multicolumn{2}{c}{HSP}  \\ 
\cline{3-10}
                               &                         & 1          & 2          & 1          & 2          & 1          & 2               & 1          & 2           \\ 
\midrule
\multirow{2}{*}{Asymm. Adv.}   & onion placement         & 304.0(1.0) & 365.7(1.0) & 295.0(1.0) & 365.9(1.0) & 296.5(1.0) & 350.7(1.0)      & 357.3(1.0) & 396.3(1.0)  \\
                               & placementdelivery       & 364.9(1.0) & 230.5(1.0) & 366.8(1.0) & 230.3(1.0) & 358.2(1.0) & 221.8(1.0)      & 371.4(1.0) & 229.9(1.0)  \\ 
\hline
\multirow{2}{*}{Coord. Ring}   & onion everywhere        & 106.0(1.0) & 112.1(1.0) & 124.6(1.0) & 123.4(1.0) & 115.7(1.0) & 118.1(1.0)      & 120.8(1.0) & 121.7(1.0)  \\
                               & dish everywhere         & 91.9(1.0)  & 97.0(1.0)  & 101.4(1.0) & 99.0(1.0)  & 107.5(1.0) & 107.1(1.0)      & 114.9(1.0) & 116.0(1.0)  \\ 
\hline
\multirow{3}{*}{Counter Circ.} & onion everywhere        & 64.80(1.0) & 62.7(1.0)  & 90.6(1.0)  & 87.4(1.0)  & 86.0(1.0)  & 78.1(1.0)       & 110.5(1.0) & 104.4(1.0)  \\
                               & dish everywhere         & 57.9(1.0)  & 56.1(1.0)  & 53.5(1.0)  & 52.5(1.0)  & 59.3(1.0)  & 55.0(1.0)       & 79.3(1.0)  & 77.8(1.0)   \\
                               & onion to middle         & 73.0(1.0)  & 72.4(1.0)  & 112.1(1.0) & 110.7(1.0) & 109.5(1.0) & 107.9(1.0)      & 149.3(1.0) & 147.1(1.0)  \\ 
\hline
\multirow{2}{*}{Distant Toma.} & tomato~placement        & (1.0)      & (1.0)      & (1.0)      & (1.0)      & (1.0)      & (1.0)           & (1.0)      & (1.0)       \\
                               & delivery                & (1.0)      & (1.0)      & (1.0)      & (1.0)      & (1.0)      & (1.0)           & (1.0)      & (1.0)       \\ 
\hline
\multirow{2}{*}{Many Ord.}     & tomato~placement        & 285.4(1.0) & 279.8(1.0) & 224.1(1.0) & 227.6(1.0) & 263.8(1.0) & 254.6(1.0)      & 315.7(1.0) & 319.9(1.0)  \\
                               & delivery                & 341.4(1.0) & 338.7(1.0) & 310.9(1.0) & 310.9(1.0) & 290.1(1.0) & 285.9(1.0)      & 379.3(1.0) & 385.2(1.0)  \\
\bottomrule
\end{tabular}
\end{table}
